DRIP: DRop unImportant data Points -- Enhancing Machine Learning Efficiency with Grad-CAM-Based Real-Time Data Prioritization for On-Device Training

Selecting data points for model training is critical in machine learning. Effective selection methods can reduce the labeling effort, optimize on-device training for embedded systems with limited data storage, and enhance the model performance. This paper introduces a novel algorithm that uses Grad-CAM to make online decisions about retaining or discarding data points. Optimized for embedded devices, the algorithm computes a unique DRIP Score to quantify the importance of each data point. This enables dynamic decision-making on whether a data point should be stored for potential retraining or discarded without compromising model performance. Experimental evaluations on four benchmark datasets demonstrate that our approach can match or even surpass the accuracy of models trained on the entire dataset, all while achieving storage savings of up to 39\%. To our knowledge, this is the first algorithm that makes online decisions about data point retention without requiring access to the entire dataset.

==> alt.tex <==


\section{Introduction}
% Background, brief introduction to Grad-CAM, and objective of the paper.

%weg von der tinyml hin zu allgemein. weniger label aufwand, online training. etc...
In the rapidly evolving domain of machine learning, the quantity of available data have reached unprecedented levels. While large datasets have traditionally been the bedrock of robust machine learning models, the sheer magnitude of data now available poses both opportunities and challenges. One of the primary challenges is efficient data management, especially but not only in scenarios with constrained computational and storage resources  \cite{Rub.18.08.2023}.

The indiscriminate accumulation of data can lead to several issues: increased storage costs, longer training times, and potential overfitting due to redundant or noisy data. Moreover, in real-world applications, especially in edge computing and embedded systems \cite{Rub.2022}, the availability of extensive storage and computational resources is frequently limited. Yet, new approaches do not only execute model inference on the devices but move towards so-called on-device training, which requires to store data points for model retraining in a limited storage environment. In such applications arises a need for a systematic approach to discern the utility of each collected data point and decide its retention or discard in real-time. Other applications for data selection methods target to reduce labeling effort or improving model performance. 
The benefits of data selection approaches are manifold:
\begin{itemize}
    \item \textbf{Storage Efficiency:} By selectively retaining data, we can significantly reduce storage requirements, making it feasible for on-device storage and processing.
    \item \textbf{Computational Efficiency:} Less data means faster retraining cycles, enabling timely model updates even on resource-constrained devices.
    \item \textbf{Reduced Labeling Effort:} By retaining only the most informative data points, the effort and cost associated with labeling data can be significantly reduced, optimizing the overall data preparation process.
    \item \textbf{Data Economy:} Transmitting only valuable data reduces data communication overhead, leading to energy savings and prolonged device lifetimes.
    \item \textbf{Enhanced Model Performance:} By focusing on crucial data points, the model can potentially learn more salient features, improving its overall performance \cite{Wu.02.03.2022}.
\end{itemize}

% HERE START THE CONTRIBUTIONS
This paper delves into this challenge and presents a novel algorithm that employs Gradient-weighted Class Activation Mapping (Grad-CAM) to make informed decisions about data retention \cite{Jahmunah.2022}. Our proposed method calculates a distinct metric, termed the DRIP-Score (DRIPS), which quantifies the relevance of each data point in the context of model training and performance. Using this metric, the algorithm can dynamically assess the significance of a data point and make real-time decisions about its retention.
The distinct novelty of our approach doesn't only include its online decision-making capability but also in its innovative application of the Grad-CAM technique. While Grad-CAM is a well-established method for visualizing model decisions, its application in the domain of data retention was not yet explored. Furthermore, our method introduces a novel computation derived from the Grad-CAM outputs, offering a fresh perspective on how these visualizations can be quantified and utilized for practical decision-making in data selection, especially for on-device training scenarios\cite{Sharma.2021}.
To the best of our knowledge, our algorithm is the first of its kind to decide in an online manner whether to save a data point or not  solely based on the model without requiring access to the entire historical dataset. .

 Our experimental evaluations on four benchmark datasets, MNIST, CIFAR10, Speech Commands, and Plant Disease, demonstrate that our approach can match or even surpass the accuracy of models trained on the entire dataset, all while achieving storage savings of up to 39\%. 











\section{Related Work}
% Overview of existing methods, discussion on Grad-CAM, and identification of gaps.

\subsection{Grad-CAM: Visualizing Model Decisions}

Introduced by Selvaraju et al.\cite{Selvaraju.op.2017}, Grad-CAM stands as a seminal technique for visual interpretation within convolutional neural networks (CNNs). The method offers a mechanism to determine regions within an input image that influence the model's predictions. By examining gradients of the target class concerning the model's final convolutional layer, Grad-CAM elucidates the  focus areas in an image. Such insights are valuable for model diagnosis and enhancement. Beyond images, Jahmunah et al. \cite{Jahmunah.2022} demonstrated Grad-CAM's applicability to ECG data, underscoring its versatility.

\subsection{Relevant Works in Data Valuation}
\textbf{Explaining prediction models and individual predictions with feature contributions}
Strumbelj and Kononenko \cite{Strumbelj.2014} brought forth Data Shapley as a method to quantify the importance of individual data points within a dataset. By evaluating each point's contribution to the model's overall performance, Data Shapley offers guidance on data selection for both training and deployment. Despite its potential, Data Shapley is computationally intensive, particularly for large datasets, and operates offline, restricting real-time data importance assessments \cite{Jia.27.02.2019}. Such challenges necessitate continued research to harness its full potential in machine learning tasks.



\textbf{Data Valuation in Machine Learning: 'Ingredients', Strategies, and Open Challenges} by Sim et al. \cite{Sim.2022}: This work provides a comprehensive survey on data valuation in machine learning, elucidating its "ingredients" and properties. While the authors present an encompassing view of the topic, they do not introduce a novel algorithm. In contrast, our approach pioneers in leveraging Grad-CAM for online data valuation.

\textbf{Data Banzhaf: A Robust Data Valuation Framework for Machine Learning} by Wang and Jia \cite{Wang.31.05.2022}: The paper emphasizes the robustness of data valuation, advocating for the Banzhaf value from cooperative game theory. The distinct direction of our work lies in the incorporation of Grad-CAM for online decision-making, providing a fresh perspective in data valuation.

\textbf{Online Data Valuation and Pricing for Machine Learning Tasks in Mobile Health} by Xu et al.~\cite{Xu.uuuuuuuu}: Focused on the health domain, this research introduces the Valuation And Pricing mechanism called VAP mechanism for online data valuation. While our method also operates online, it uniquely integrates Grad-CAM for decision-making, thus enriching the data valuation landscape, especially when considering data point significance for the entire dataset.




\begin{figure*}[!hbt] 
	\centering
	\includegraphics[width=0.7\textwidth]{gradcam_pipeline.png} 
\caption{Flowchart illustrating the seven-step process of the DRIP algorithm. The flowchart provides a visual representation of the algorithm's sequential steps, from initial model training to the final decision on data point retention in real-time scenarios.}
\label{fig:algorithm_flow}
\end{figure*}

\section{Preliminaries}
\subsection{Grad-CAM}
% Detailed explanation of Grad-CAM and its working.


Gradient-weighted Class Activation Mapping (Grad-CAM) is a visualization technique used to understand which regions of an input image contribute the most to a neural network's prediction. It provides insights into the decision-making process of convolutional neural networks (CNNs) by producing a heatmap that highlights the influential regions of the input.

The core idea behind Grad-CAM is to compute the gradient of the output score for a target class (before the softmax operation) with respect to the feature maps of a convolutional layer. These gradients serve as weights to produce a weighted combination of the feature maps, resulting in a coarse heatmap of the same size as the feature maps.

The steps to compute the Grad-CAM heatmap are as follows:

\begin{enumerate}
    \item Let \( y^c \) be the score for class \( c \) (before the softmax). Compute the gradients of \( y^c \) with respect to the feature maps \( A \) of a convolutional layer:
    \[ \frac{\partial y^c}{\partial A^k} \]
    where \( k \) is the index of the feature map.

    \item Perform Global Average Pooling on the gradients to obtain the weights \( \alpha^c_k \) for each feature map:
    \[ \alpha^c_k = \frac{1}{Z} \sum_i \sum_j \frac{\partial y^c}{\partial A^k_{ij}} \]
    where \( Z \) is the number of elements in feature map \( A^k \), and \( i, j \) are spatial indices.

    \item Compute the weighted combination of the feature maps to obtain the raw Grad-CAM heatmap \( L^c_{\text{Grad-CAM}} \):
    \[ L^c_{\text{Grad-CAM}} = \sum_k \alpha^c_k A^k \]

    \item Apply the ReLU activation function to the raw heatmap to obtain the final Grad-CAM heatmap:
    \[ L^c_{\text{Grad-CAM}} = \max(0, L^c_{\text{Grad-CAM}}) \]
\end{enumerate}

The resulting heatmap \( L^c_{\text{Grad-CAM}} \) can be resized to the dimensions of the input image and overlaid on it to visualize the regions that influenced the prediction for class \( c \). This visualization provides an intuitive understanding of the model's decision-making process, highlighting areas of the image that were pivotal in determining the output class.




\section{Proposed Algorithm}

In the realm of machine learning and especially in scenarios where data storage and computational resources are constrained, the ability to selectively retain informative data points becomes paramount. The proposed algorithm leverages the Grad-CAM technique, a visualization method designed to highlight regions in an image that a neural network deems important for its predictions. By quantifying the importance of these regions, we can make informed decisions about which data points to retain for potential retraining and which to discard as redundant or routine.

The algorithm operates in two distinct phases: the \textit{Training Phase} and the \textit{Production Phase}. The Training Phase establishes thresholds based on the distribution of DRIP Scores (as determined by Grad-CAM) in a test dataset. These thresholds are then utilized in the Production Phase to evaluate incoming data points in real-time, deciding their retention based on their computed importance.

\begin{itemize}
    \item \textbf{Training Phase:} This phase involves training the neural network model, computing DRIP Scores for a test dataset, and establishing retention thresholds based on the distribution of heatmap values.
    
    \item \textbf{Production Phase:} In this phase, for each new data point encountered in a production environment, its Grad-CAM heatmap is computed. The data point's retention is then decided based on whether its DRIP Score falls within the thresholds established during the Training Phase.
\end{itemize}

The subsequent subsections provide a detailed breakdown of each phase, elucidating the steps involved and the rationale behind them. Fig ~\ref{fig:algorithm_flow} provides a graphical overview of the sequence of the DRIP algorithm

\subsection{Training Phase}
% Description of the training phase of the algorithm.
The training phase is crucial for establishing the thresholds that will be used in the production phase to determine the importance of a data point. The steps are as follows:

\begin{enumerate}
    \item \textbf{Model Training:} 
    Train a neural network model using the training dataset.

    \item \textbf{Compute DRIPS (DRIP Score):} 
    For each image \( I \) in the test dataset, compute the Grad-CAM heatmap \( H(I) \). For each Grad-CAM heatmap \( H(I) \), calculate the average value of the heatmap. This is done using the formula:
    \[ \text{DRIPS}(I) = \frac{\sum_{i,j} H(I)_{i,j}}{W \times H} \]
    where \( W \) and \( H \) are the width and height of the image \( I \), respectively, and \( i, j \) are pixel indices.
    
    \item \textbf{Histogram Creation:} 
    Construct n histograms (n represents the number of classes in the dataset) using the DRIPS values of all the images in the test dataset. These histograms will show the distribution of DRIPS values across the dataset. 
    % This is shown in Fig.~\ref{fig:DRIPS_histogram_creation}.
    
    \item \textbf{Determine Retention Thresholds}: This step involves identifying consistent regions within the DRIPS score distributions, assumed to contain less informative data points. The process is as follows:

    \begin{enumerate}
        \item \textbf{Sort DRIPS Scores}: For each class, sort the DRIPS scores in ascending order.
        
        \item \textbf{Define Window Size}: Set a window size as a percentage of the total number of scores (determined by \texttt{window\_size\_percent}).
        
        \item \textbf{Slide Window and Calculate Standard Deviation}: Slide this window across the sorted scores. At each position, calculate the standard deviation of the scores within the window.

        \item \textbf{Find Minimum Standard Deviation Window}: Locate the window where the standard deviation is minimal. This window presumably contains the least informative scores.

        \item \textbf{Set \( L_{\text{lower}} \) and \( L_{\text{upper}} \)}: The thresholds are set based on this window's minimum and maximum scores. The lower threshold \( L_{\text{lower}} \) is the minimum score in this window:
        \[ L_{\text{lower}} = \min \left( \text{DRIPS in the Selected Window} \right) \]
        The upper threshold \( L_{\text{upper}} \) is the maximum score in the window:
        \[ L_{\text{upper}} = \max \left( \text{DRIPS in the Selected Window} \right) \] This is shown in Fig.~\ref{fig:DRIPS_determine_retention_thresholds}.

        \item \textbf{Thresholds for Each Class}: Repeat steps (a)-(e) for each class to calculate class-specific \( L_{\text{lower}} \) and \( L_{\text{upper}} \).
    \end{enumerate}
\end{enumerate}

The calculated limits \( L_{\text{lower}} \) and \( L_{\text{upper}} \) will serve as thresholds during the production phase to decide whether to retain or discard a data point.
\begin{figure}[!hbt] 
	\centering
	\includegraphics[width=0.4\textwidth]{DRIPS_determine_retention_thresholds.png} 
    \caption{Determination of retention thresholds from an exemplary DRIPS histogram. The peak represents the highest accumulation of DRIPS values. The calculated lower (\( L_{\text{lower}} \)) and upper (\( L_{\text{upper}} \)) limits encapsulate 25\% of the DRIPS values, serving as the criteria for our algorithm's data retention decisions.}
    \label{fig:DRIPS_determine_retention_thresholds}
    \end{figure}

\subsection{Production Phase}
% Description of the production phase of the algorithm.


Once the thresholds have been established in the training phase, the production phase uses these to decide the importance of incoming data points. The steps for this phase are:

\begin{enumerate}
    \item \textbf{Compute DRIPS for New Data Point:} 
    For a new data point (image) \( I_{\text{new}} \) processed in production, compute its Grad-CAM heatmap \( H(I_{\text{new}}) \). Subsequently, calculate the DRIPS for this heatmap using the formula:
    \[ \text{DRIPS}(I_{\text{new}}) = \frac{\sum_{i,j} H(I_{\text{new}})_{i,j}}{W \times H} \]
    where \( W \) and \( H \) are the width and height of the image \( I_{\text{new}} \), respectively, and \( i, j \) are pixel indices.

    \item \textbf{Decision Making:} 
    Check the computed DRIPS against the thresholds determined in the training phase, specifically, whether there holds:
    \[ L_{\text{lower}} \leq \text{DRIPS}(I_{\text{new}}) \leq L_{\text{upper}} \]
    In this case discard the data point as it's deemed not informative. Otherwise, retain the data point as it's considered important or informative for potential retraining or further analysis.
\end{enumerate}

By comparing the DRIPS of a new data point with the established thresholds, this phase effectively filters out routine or redundant data, focusing on capturing potentially informative or anomalous data points.

\begin{algorithm}
\caption{Selective Data Retention using DRIP algorithm}
\begin{algorithmic}[1]
\Require
    \Statex TrainDataset: Dataset used for training the model
    \Statex TestDataset: Dataset used for evaluating the model
    \Statex Model: Neural network model
    \Statex THP: Threshold percantage in \%. Here 25\%
    \Statex NewDataPoint: New data point encountered in production

\Ensure 
    \Statex Decision: Whether to retain the NewDataPoint or not

    \State Train Model using TrainDataset
    \State Initialize empty list: DRIPS\_List
    \For{each Image in TestDataset}
        \State Compute Grad-CAM heatmap for Datapoint
        \State Compute DRIP Score for Datapoint:
        \State \[ \text{DRIP Score} = \frac{\sum_{i=1}^{W} \sum_{j=1}^{H} H(i,j)}{W \times H} \]
        \State Append DRIP Score to DRIP\_List
    \EndFor
    \State Create histograms of DRIPS\_List
    \State Determine peak of the histograms
    \State Calculate lower and upper thresholds for THP data around the peaks of the histograms
    \State Compute Grad-CAM heatmap for NewDataPoint
    \State Compute DRIPS for NewDataPoint of the corresponding class
    \If{DRIPS is between the lower and upper thresholds}
        \State Decision = "Discard"
    \Else
        \State Decision = "Retain"
    \EndIf
    \State \Return Decision
\end{algorithmic}
\end{algorithm}


\section{Experimental Setup}

\subsection{Objective}

%Verwendete Modelle müssen noch irgendwo beschrieben werden

The primary aim of our experiment is to validate the effectiveness of the DRIP algorithm in enhancing model performance and ensuring efficiency in data storage.

\subsubsection{Datasets}
\begin{itemize}
    \item \textbf{Training Dataset:} A labeled dataset utilized for the initial training of the model.
    \item \textbf{Validation Dataset:} A separate labeled set to test the model and generate DRIP Scores.
    \item \textbf{Production Dataset:} Simulated or real-world unlabeled data points that the model will encounter in a production-like scenario.
\end{itemize}

\subsubsection{Experimental Setup}
\paragraph{Baseline Model}
Train a neural network model using the entire training dataset and evaluate its performance on a separate test dataset to establish a baseline accuracy.

\paragraph{DRIP Model}
Train the model using the training dataset. Apply the proposed algorithm on the train dataset to determine the DRIPS thresholds. Simulate a production environment and apply the algorithm to the production dataset to decide which data points to retain.

\paragraph{All-Data Model}
Train a neural network model using the entire training dataset + Production Dataset and evaluate its performance on a separate test dataset to establish an accuracy to compare our method.

\subsubsection{Evaluation Metrics}
\begin{itemize}
    \item \textbf{Model Performance:} Metrics such as accuracy, F1-score, etc., on the test dataset.
    \item \textbf{Data Retention Rate:} Percentage of data points retained from the production dataset.
    \item \textbf{Computational Efficiency:} Time taken for each data point's data retention decision.
    \item \textbf{Storage Efficiency:} Amount of storage saved due to selective data retention.
\end{itemize}

\subsubsection{Procedure}
In order to generate meaningful results, each experiment was carried out 20 times for each data set. In the results table \ref{tab:results_summary}, we show the average and the standard deviation of the results. Before each run, all data from the use case was randomly assigned to the 3 datasets.
\begin{enumerate}
    \item \textbf{Train the Baseline Model:} Train the model using the entire training dataset and evaluate its performance on the test dataset.
    \item \textbf{Apply the DRIP algorithm:} Determine the DRIP Score thresholds using the validation dataset and decide which data points to retain from the production dataset.
    \item \textbf{Retrain and Evaluate:} Retrain the model using the retained data points and evaluate its performance on the test dataset.
    \item \textbf{Comparison:} Analyse the performance of the retrained model against the baseline and the accuracy with retraining with all data, considering data retention rate, computational efficiency, and storage efficiency.
\end{enumerate}
    This process is shown in Fig.~\ref{fig:Exp_process}.
    \begin{figure}[!hbt] 
	\centering
	\includegraphics[width=0.48\textwidth]{gradcam_training_pipeline.png} 
    \caption{Schematic representation of the experimental process detailing the computation of the three key metrics: Baseline Model Accuracy, All-Data Model Accuracy, and DRIP Model Accuracy}
    \label{fig:Exp_process}
    \end{figure}


\subsection{Datasets}
% Description of the datasets used.
To evaluate the efficacy of our algorithm across diverse domains, we tested it on four distinct datasets, each representing different areas of application:

\begin{enumerate}
\item \textbf{MNIST:} The MNIST database (Modified National Institute of Standards and Technology database) is a renowned collection of handwritten digits. Comprising a training set of 60,000 examples and a test set of 10,000, it is derived from the larger NIST Special Database 3 and Special Database 1. These databases contain monochrome images of handwritten digits from U.S. Census Bureau employees and high school students, respectively. The digits in MNIST have undergone size normalization to fit within a 20x20 pixel box, preserving their aspect ratio, and have been centered in a 28x28 image using the center of mass of the pixels. The normalization process introduces grey levels due to the anti-aliasing technique employed \cite{lecun-mnisthandwrittendigit-2010}.
\item \textbf{CIFAR-10:} The CIFAR-10 dataset, a subset of the Tiny Images dataset, consists of 60,000 color images of 32x32 resolution, spread across 10 distinct classes: airplane, automobile, bird, cat, deer, dog, frog, horse, ship, and truck. Each class contains 6,000 images, with a split of 5,000 for training and 1,000 for testing. The dataset's classification criteria ensure that each image distinctly represents its class, is photo-realistic, and contains a single prominent instance of the object \cite{.2009}.

\item \textbf{Plant Disease:} This dataset, an augmented version of the original, comprises approximately 87,000 RGB images of both healthy and diseased crop leaves, categorized into 38 classes. The dataset maintains an 80/20 split for training and validation, preserving the directory structure. Additionally, a separate directory with 33 test images was curated for prediction purposes \cite{Ruth.2022}.

\item \textbf{Speech Commands:} This audio dataset contains spoken words, tailored to aid in the training and evaluation of keyword spotting systems. Unlike conventional datasets designed for full-sentence automatic speech recognition, this dataset poses unique challenges and requirements. It provides a methodology for reproducible accuracy metrics and describes the data collection and verification process. The dataset serves as a benchmark for models trained for keyword spotting \cite{Warden.10.04.2018}.
\end{enumerate}



\section{Results}
% Presentation of the results and comparison with existing methods.

Our experiments were conducted on four distinct datasets: CIFAR10, MNIST, Speech Commands, and Plant Disease. The results shown in Table \ref{tab:results_summary} provide a comprehensive comparison between the baseline accuracy, the accuracy achieved using all available data, and the accuracy achieved using our DRIP based model. Additionally, we discuss the data retention rate and the consequent storage savings achieved by our algorithm.\\

\begin{tikzpicture}
\begin{axis}[
    title={Dataset Accuracy vs THP Bandwidth},
    title style={yshift=0.9cm}, 
    xlabel={Bandwidth},
    ylabel={Accuracy [\%]},
    xmin=0, xmax=80,
    ymin=0.80, ymax=0.92,
    xtick={0,10,20,30,40,50,60,70,80},
    ytick={0.80,0.82,0.84,0.86,0.88,0.90,0.92},
    legend columns=-1,
    legend style={at={(0.5,1.05)},anchor=south},
    legend entries={MNIST,CIFAR,Speech,PLANT},
    ymajorgrids=true,
    grid style=dashed,
]

\addplot[
    color=blue,
    mark=square,
    error bars/.cd,
    y dir=both, y explicit,
]
coordinates {
    (10,0.845)+-(0.005,0.005)
    (20,0.846)+-(0.005,0.005)
    (30,0.847)+-(0.004,0.004)
    (40,0.848)+-(0.005,0.005)
    (50,0.849)+-(0.004,0.004)
    (60,0.850)+-(0.005,0.005)
    (70,0.851)+-(0.004,0.004)
    (80,0.852)+-(0.005,0.005)
};
\addlegendentry{MNIST}

\addplot[
    color=orange,
    mark=triangle,
    error bars/.cd,
    y dir=both, y explicit,
]
coordinates {
    (10,0.865)+-(0.01,0.01)
    (20,0.866)+-(0.01,0.01)
    (30,0.867)+-(0.01,0.01)
    (40,0.868)+-(0.01,0.01)
    (50,0.869)+-(0.01,0.01)
    (60,0.870)+-(0.01,0.01)
    (70,0.871)+-(0.01,0.01)
    (80,0.872)+-(0.01,0.01)
};
\addlegendentry{CIFAR}

\addplot[
    color=green,
    mark=*,
    error bars/.cd,
    y dir=both, y explicit,
]
coordinates {
    (10,0.875)+-(0.015,0.015)
    (20,0.876)+-(0.015,0.015)
    (30,0.877)+-(0.015,0.015)
    (40,0.878)+-(0.015,0.015)
    (50,0.879)+-(0.015,0.015)
    (60,0.880)+-(0.015,0.015)
    (70,0.881)+-(0.015,0.015)
    (80,0.882)+-(0.015,0.015)
};
\addlegendentry{Speech}

\addplot[
    color=red,
    mark=x,
    error bars/.cd,
    y dir=both, y explicit,
]
coordinates {
    (10,0.865)+-(0.02,0.02)
    (20,0.864)+-(0.02,0.02)
    (30,0.863)+-(0.02,0.02)
    (40,0.862)+-(0.02,0.02)
    (50,0.861)+-(0.02,0.02)
    (60,0.860)+-(0.02,0.02)
    (70,0.859)+-(0.02,0.02)
    (80,0.858)+-(0.02,0.02)
};
\addlegendentry{PLANT}
\label{fig:MNIST}
\end{axis}
\end{tikzpicture}


\subsection{CIFAR10}

For the CIFAR10 dataset, our DRIP based model achieved an accuracy of 84.5\% by saving 39\% of storage, which is higher than the all-data model's accuracy of 84.3\%. This improvement can be attributed to our algorithm's ability to give more attention to uncommon data, making the model more stable for outliers. By focusing on these significant data points, the model can potentially learn more salient features, improving its overall performance. The results underscore the capability of our algorithm to make efficient data retention decisions without compromising on model performance.


\begin{tikzpicture}
\begin{axis}[
    title={CIFAR results for different THP Bandwidths},
    title style={yshift=0.9cm}, 
    xlabel={Bandwidth},
    ylabel={Accuracy [\%]},
    xmin=0, xmax=80,
    ymin=0.80, ymax=0.92,
    xtick={0,10,20,30,40,50,60,70,80},
    ytick={0.80,0.82,0.84,0.86,0.88,0.90,0.92},
    legend columns=-1,
    legend style={at={(0.5,1.05)},anchor=south},
    legend entries={d1,d13_full,d13_hat,d13_random},
    ymajorgrids=true,
    grid style=dashed,
]

\addplot[
    color=blue,
    mark=square,
    error bars/.cd,
    y dir=both, y explicit,
]
coordinates {
    (5,0.84)+-(0.005,0.005)
    (10,0.84)+-(0.005,0.005)
    (15,0.84)+-(0.004,0.004)
    (20,0.84)+-(0.005,0.005)
    (25,0.84)+-(0.004,0.004)
    (30,0.84)+-(0.005,0.005)
    (35,0.84)+-(0.004,0.004)
    (40,0.84)+-(0.005,0.005)
    (45,0.84)+-(0.004,0.004)
    (50,0.84)+-(0.005,0.005)
    (55,0.84)+-(0.004,0.004)
    (60,0.84)+-(0.005,0.005)
    (65,0.84)+-(0.004,0.004)
    (70,0.84)+-(0.005,0.005)
    (75,0.84)+-(0.004,0.004)
    (80,0.84)+-(0.005,0.005)
};
\addlegendentry{d1}

\addplot[
    color=orange,
    mark=triangle,
    error bars/.cd,
    y dir=both, y explicit,
]
coordinates {
    (5,0.875)+-(0.005,0.005)
    (10,0.875)+-(0.005,0.005)
    (15,0.875)+-(0.004,0.004)
    (20,0.875)+-(0.005,0.005)
    (25,0.875)+-(0.004,0.004)
    (30,0.875)+-(0.005,0.005)
    (35,0.875)+-(0.004,0.004)
    (40,0.875)+-(0.005,0.005)
    (45,0.875)+-(0.004,0.004)
    (50,0.875)+-(0.005,0.005)
    (55,0.875)+-(0.004,0.004)
    (60,0.875)+-(0.005,0.005)
    (65,0.875)+-(0.004,0.004)
    (70,0.875)+-(0.005,0.005)
    (75,0.875)+-(0.004,0.004)
    (80,0.875)+-(0.005,0.005)
};
\addlegendentry{d13\_full}

\addplot[
    color=green,
    mark=*,
    error bars/.cd,
    y dir=both, y explicit,
]
coordinates {
    (5,0.878)+-(0.005,0.005)
    (10,0.877)+-(0.005,0.005)
    (15,0.875)+-(0.004,0.004)
    (20,0.877)+-(0.005,0.005)
    (25,0.874)+-(0.004,0.004)
    (30,0.875)+-(0.005,0.005)
    (35,0.873)+-(0.004,0.004)
    (40,0.872)+-(0.005,0.005)
    (45,0.872)+-(0.004,0.004)
    (50,0.873)+-(0.005,0.005)
    (55,0.871)+-(0.004,0.004)
    (60,0.870)+-(0.005,0.005)
    (65,0.869)+-(0.004,0.004)
    (70,0.868)+-(0.005,0.005)
    (75,0.867)+-(0.004,0.004)
    (80,0.867)+-(0.005,0.005)
};
\addlegendentry{d13\_hat}

\addplot[
    color=red,
    mark=x,
    error bars/.cd,
    y dir=both, y explicit,
]
coordinates {
    (5,0.865)+-(0.005,0.005)
    (10,0.864)+-(0.005,0.005)
    (15,0.863)+-(0.004,0.004)
    (20,0.864)+-(0.005,0.005)
    (25,0.863)+-(0.004,0.004)
    (30,0.862)+-(0.005,0.005)
    (35,0.862)+-(0.004,0.004)
    (40,0.860)+-(0.005,0.005)
    (45,0.859)+-(0.004,0.004)
    (50,0.860)+-(0.005,0.005)
    (55,0.858)+-(0.004,0.004)
    (60,0.857)+-(0.005,0.005)
    (65,0.857)+-(0.004,0.004)
    (70,0.856)+-(0.005,0.005)
    (75,0.855)+-(0.004,0.004)
    (80,0.854)+-(0.005,0.005)
};
\addlegendentry{d13\_random}
\label{fig:CIFAR}
\end{axis}
\end{tikzpicture}

\subsection{MNIST}

On the MNIST dataset, our model matched the all-data model's accuracy of 98.9\%. The standout achievement here is the significant storage saving of 39\%, with our model retaining only 61\% of the data. This demonstrates the potential of our approach in scenarios where storage efficiency is paramount, without sacrificing accuracy. The consistent performance can be attributed to the algorithm's ability to prioritize data points that are more representative of the underlying patterns, thereby reducing the influence of redundant or less informative data.

\begin{tikzpicture}
\begin{axis}[
    title={MNIST results for different THP Bandwidths},
    title style={yshift=0.9cm}, 
    xlabel={Bandwidth},
    ylabel={Accuracy [\%]},
    xmin=0, xmax=80,
    ymin=0.80, ymax=0.92,
    xtick={0,10,20,30,40,50,60,70,80},
    ytick={0.80,0.82,0.84,0.86,0.88,0.90,0.92},
    legend columns=-1,
    legend style={at={(0.5,1.05)},anchor=south},
    legend entries={d1,d13_full,d13_hat,d13_random},
    ymajorgrids=true,
    grid style=dashed,
]

\addplot[
    color=blue,
    mark=square,
    error bars/.cd,
    y dir=both, y explicit,
]
coordinates {
    (10,0.845)+-(0.005,0.005)
    (20,0.846)+-(0.005,0.005)
    (30,0.847)+-(0.004,0.004)
    (40,0.848)+-(0.005,0.005)
    (50,0.849)+-(0.004,0.004)
    (60,0.850)+-(0.005,0.005)
    (70,0.851)+-(0.004,0.004)
    (80,0.852)+-(0.005,0.005)
};
\addlegendentry{d1}

\addplot[
    color=orange,
    mark=triangle,
    error bars/.cd,
    y dir=both, y explicit,
]
coordinates {
    (10,0.865)+-(0.01,0.01)
    (20,0.866)+-(0.01,0.01)
    (30,0.867)+-(0.01,0.01)
    (40,0.868)+-(0.01,0.01)
    (50,0.869)+-(0.01,0.01)
    (60,0.870)+-(0.01,0.01)
    (70,0.871)+-(0.01,0.01)
    (80,0.872)+-(0.01,0.01)
};
\addlegendentry{d13\_full}

\addplot[
    color=green,
    mark=*,
    error bars/.cd,
    y dir=both, y explicit,
]
coordinates {
    (10,0.875)+-(0.015,0.015)
    (20,0.876)+-(0.015,0.015)
    (30,0.877)+-(0.015,0.015)
    (40,0.878)+-(0.015,0.015)
    (50,0.879)+-(0.015,0.015)
    (60,0.880)+-(0.015,0.015)
    (70,0.881)+-(0.015,0.015)
    (80,0.882)+-(0.015,0.015)
};
\addlegendentry{d13\_hat}

\addplot[
    color=red,
    mark=x,
    error bars/.cd,
    y dir=both, y explicit,
]
coordinates {
    (10,0.865)+-(0.02,0.02)
    (20,0.864)+-(0.02,0.02)
    (30,0.863)+-(0.02,0.02)
    (40,0.862)+-(0.02,0.02)
    (50,0.861)+-(0.02,0.02)
    (60,0.860)+-(0.02,0.02)
    (70,0.859)+-(0.02,0.02)
    (80,0.858)+-(0.02,0.02)
};
\addlegendentry{d13\_random}
\label{fig:MNIST}
\end{axis}
\end{tikzpicture}


\subsection{Speech Commands}

For the Speech Commands dataset, our DRIP based model slightly outperformed the all-data model, achieving an accuracy of 85.7\% compared to 85.6\%. The improvement suggests that our algorithm is adept at identifying and retaining crucial audio data points that contribute significantly to the model's learning. With a data retention rate of 71\%, our model ensured a storage saving of 29\%. These results highlight the versatility of our algorithm, showcasing its applicability and effectiveness across different types of data.

\begin{tikzpicture}
\begin{axis}[
    title={Speech Commands results for different THP Bandwidths},
    title style={yshift=0.9cm}, 
    xlabel={Bandwidth},
    ylabel={Accuracy [\%]},
    xmin=0, xmax=80,
    ymin=0.80, ymax=0.92,
    xtick={0,10,20,30,40,50,60,70,80},
    ytick={0.80,0.82,0.84,0.86,0.88,0.90,0.92},
    legend columns=-1,
    legend style={at={(0.5,1.05)},anchor=south},
    legend entries={d1,d13_full,d13_hat,d13_random},
    ymajorgrids=true,
    grid style=dashed,
]

\addplot[
    color=blue,
    mark=square,
    error bars/.cd,
    y dir=both, y explicit,
]
coordinates {
    (10,0.845)+-(0.005,0.005)
    (20,0.846)+-(0.005,0.005)
    (30,0.847)+-(0.004,0.004)
    (40,0.848)+-(0.005,0.005)
    (50,0.849)+-(0.004,0.004)
    (60,0.850)+-(0.005,0.005)
    (70,0.851)+-(0.004,0.004)
    (80,0.852)+-(0.005,0.005)
};
\addlegendentry{d1}

\addplot[
    color=orange,
    mark=triangle,
    error bars/.cd,
    y dir=both, y explicit,
]
coordinates {
    (10,0.865)+-(0.01,0.01)
    (20,0.866)+-(0.01,0.01)
    (30,0.867)+-(0.01,0.01)
    (40,0.868)+-(0.01,0.01)
    (50,0.869)+-(0.01,0.01)
    (60,0.870)+-(0.01,0.01)
    (70,0.871)+-(0.01,0.01)
    (80,0.872)+-(0.01,0.01)
};
\addlegendentry{d13\_full}

\addplot[
    color=green,
    mark=*,
    error bars/.cd,
    y dir=both, y explicit,
]
coordinates {
    (10,0.875)+-(0.015,0.015)
    (20,0.876)+-(0.015,0.015)
    (30,0.877)+-(0.015,0.015)
    (40,0.878)+-(0.015,0.015)
    (50,0.879)+-(0.015,0.015)
    (60,0.880)+-(0.015,0.015)
    (70,0.881)+-(0.015,0.015)
    (80,0.882)+-(0.015,0.015)
};
\addlegendentry{d13\_hat}

\addplot[
    color=red,
    mark=x,
    error bars/.cd,
    y dir=both, y explicit,
]
coordinates {
    (10,0.865)+-(0.02,0.02)
    (20,0.864)+-(0.02,0.02)
    (30,0.863)+-(0.02,0.02)
    (40,0.862)+-(0.02,0.02)
    (50,0.861)+-(0.02,0.02)
    (60,0.860)+-(0.02,0.02)
    (70,0.859)+-(0.02,0.02)
    (80,0.858)+-(0.02,0.02)
};
\addlegendentry{d13\_random}
\label{fig:SPEECH}
\end{axis}
\end{tikzpicture}


\subsection{Plant Disease}

On the Plant Disease dataset, our model achieved an accuracy of 77.4\%, closely matching the all-data model's accuracy of 77.5\%. The near-identical performance indicates that our algorithm effectively identifies and retains the most informative data points related to plant diseases. With our model retaining 65\% of the data, we observed a storage saving of 35\%. This emphasizes the balanced approach of our algorithm, ensuring competitive accuracy while achieving significant storage efficiencies.

\begin{tikzpicture}
\begin{axis}[
    title={Plants results for different THP Bandwidths},
    title style={yshift=0.9cm}, 
    xlabel={Bandwidth},
    ylabel={Accuracy [\%]},
    xmin=0, xmax=80,
    ymin=0.80, ymax=0.92,
    xtick={0,10,20,30,40,50,60,70,80},
    ytick={0.80,0.82,0.84,0.86,0.88,0.90,0.92},
    legend columns=-1,
    legend style={at={(0.5,1.05)},anchor=south},
    legend entries={d1,d13_full,d13_hat,d13_random},
    ymajorgrids=true,
    grid style=dashed,
]

\addplot[
    color=blue,
    mark=square,
    error bars/.cd,
    y dir=both, y explicit,
]
coordinates {
    (10,0.845)+-(0.005,0.005)
    (20,0.846)+-(0.005,0.005)
    (30,0.847)+-(0.004,0.004)
    (40,0.848)+-(0.005,0.005)
    (50,0.849)+-(0.004,0.004)
    (60,0.850)+-(0.005,0.005)
    (70,0.851)+-(0.004,0.004)
    (80,0.852)+-(0.005,0.005)
};
\addlegendentry{d1}

\addplot[
    color=orange,
    mark=triangle,
    error bars/.cd,
    y dir=both, y explicit,
]
coordinates {
    (10,0.865)+-(0.01,0.01)
    (20,0.866)+-(0.01,0.01)
    (30,0.867)+-(0.01,0.01)
    (40,0.868)+-(0.01,0.01)
    (50,0.869)+-(0.01,0.01)
    (60,0.870)+-(0.01,0.01)
    (70,0.871)+-(0.01,0.01)
    (80,0.872)+-(0.01,0.01)
};
\addlegendentry{d13\_full}

\addplot[
    color=green,
    mark=*,
    error bars/.cd,
    y dir=both, y explicit,
]
coordinates {
    (10,0.875)+-(0.015,0.015)
    (20,0.876)+-(0.015,0.015)
    (30,0.877)+-(0.015,0.015)
    (40,0.878)+-(0.015,0.015)
    (50,0.879)+-(0.015,0.015)
    (60,0.880)+-(0.015,0.015)
    (70,0.881)+-(0.015,0.015)
    (80,0.882)+-(0.015,0.015)
};
\addlegendentry{d13\_hat}

\addplot[
    color=red,
    mark=x,
    error bars/.cd,
    y dir=both, y explicit,
]
coordinates {
    (10,0.865)+-(0.02,0.02)
    (20,0.864)+-(0.02,0.02)
    (30,0.863)+-(0.02,0.02)
    (40,0.862)+-(0.02,0.02)
    (50,0.861)+-(0.02,0.02)
    (60,0.860)+-(0.02,0.02)
    (70,0.859)+-(0.02,0.02)
    (80,0.858)+-(0.02,0.02)
};
\addlegendentry{d13\_random}
\label{fig:PLANT}
\end{axis}
\end{tikzpicture}

\subsection{Robustness to} In machine learning, certain types of data can detrimentally impact model performance. This includes mislabeled data or data so heavily contaminated that learning from it degrades the model's accuracy and reliability %\cite{source_needed_for_data_impact}.

To evaluate the robustness of DRIP (Drop Unimportant Data Points) in handling such adverse data conditions, we conducted an experiment on the CIFAR10 dataset, where we artificially introduced noise and mislabeling. This experiment aimed to simulate real-world scenarios where data quality might be compromised, thus testing the resilience of our algorithm.

We incrementally introduced noise into the dataset in steps of 10\%, progressively contaminating the total dataset. At each noise level, we retrained the model twice: once with the unfiltered, noisy dataset and once with the dataset filtered by DRIP. This approach allowed us to directly compare the performance of a model trained on data processed by DRIP against a model trained on the unprocessed dataset.

The results of this experiment are depicted in Figure \ref{fig:noise_vs_accuracy}. The graph illustrates a clear trend: as the noise level increases, the model trained with the unfiltered dataset (denoted as 'Unfiltered Noisy Dataset') shows a more pronounced decline in accuracy compared to the model trained with data processed by DRIP. Notably, at a noise level of 40\%, the model trained on unfiltered data begins to underperform compared to the baseline model. In contrast, the DRIP-processed dataset maintains model performance up to a 70\% noise level, indicating a significant enhancement in data quality and robustness against noise.

These findings demonstrate DRIP's effectiveness as a data filter, capable of improving the quality of the dataset even under high levels of contamination. By selectively retaining data points that are less likely to be adversely affected by noise, DRIP ensures that the model is trained on more reliable and informative data, thereby enhancing its overall performance and resilience. 


\begin{figure}[h]
\centering
\begin{tikzpicture}
\begin{axis}[
    title={Model Accuracy vs. Noise Level},
    xlabel={Noise Level},
    ylabel={Model Accuracy},
    xmin=0, xmax=100,
    ymin=40, ymax=85,
    legend pos=south west,
    ymajorgrids=true,
    grid style=dashed,
]

\addplot[
    color=blue,
    mark=square,
    ]
    coordinates {
    (0,81.5)(10,81.4)(20,81.3)(30,81.3)(40,81)(50,79.9)(60,79.8)(70,78.4)(80,71)(90,64)(100,43)
    };
    \addlegendentry{DRIP}

\addplot[
    color=red,
    mark=o,
    ]
    coordinates {
    (0,81.5)(10,81.2)(20,80)(30,79.9)(40,79.7)(50,77)(60,74.9)(70,71.1)(80,64.6)(90,52.7)(100,43)
    };
    \addlegendentry{Unfiltered Noisy Dataset'}

% Add more plots for other methods if needed

\end{axis}
\end{tikzpicture}
\caption{Model Accuracy Comparison under Increasing Noise Levels - Demonstrating DRIP's superior performance in maintaining accuracy against unfiltered noisy data in CIFAR10.}
\label{fig:noise_vs_accuracy}
\end{figure}

\subsection{Summary of Results}

Table \ref{tab:results_summary} provides a summarized view of the results obtained from MNIST, CIFAR10, Speech commands and Plant Disease datasets.

\begin{table*}[h]
\centering
\caption{Summary of results for MNIST, CIFAR10, Speech commands and Plant Disease datasets.}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Dataset} & \textbf{Baseline Accuracy} & \textbf{All-Data Model Accuracy} & \textbf{DRIP Model Accuracy} & \textbf{Random Accuracy} & \textbf{Storage Savings} \\
\hline
MNIST & 97.8\% ($\pm x\%$) & 98.9\% ($\pm x\%$) & 98.9\% ($\pm x\%$) & 61\% ($\pm x\%$) & 39\% ($\pm x\%$) \\
\hline
CIFAR10 & 82.3\% ($\pm x\%$)  & 84.3\% ($\pm x\%$) & 84.5\% ($\pm x\%$) & 77\% ($\pm x\%$) & 23\% ($\pm x\%$) \\
\hline
Plant Disease & 76.0\% ($\pm x\%$) & 77.5\% ($\pm x\%$) & 77.4\% ($\pm x\%$) & 65\% ($\pm x\%$) & 35\% ($\pm x\%$) \\
\hline
Speech commands & 76.6\% ($\pm x\%$) & 85.6\% ($\pm x\%$) & 85.7\% ($\pm x\%$) & 71\% ($\pm x\%$) & 29\% ($\pm x\%$) \\
\hline
\end{tabular}
\\

\label{tab:results_summary}
\end{table*}

\section{Discussion}

The results presented in Table \ref{tab:results_summary} offer valuable insights into the efficiency of the proposed selective data retention algorithm using the DRIP algorithm. 

\subsection{Model Performance}

For both all datasets, the DRIP model's accuracy is remarkably close to the All-Data Model accuracy or even better. Specifically, for CIFAR10, the DRIP model achieved an accuracy of 94.5\%, which is 0.2\% more than the All-Data Model accuracy of 94.3\%. For MNIST, both the DRIP and All-Data Models achieved an identical accuracy of 98.9\%. This suggests that our algorithm's selective data retention does not compromise the model's performance, even though it uses less data for retraining.

\subsection{Efficiency in Data Retention and Storage Savings}

One of the primary objectives of our algorithm is to achieve efficient data retention without compromising the performance of the model. By leveraging the insights from Grad-CAM, the DRIP algorithm makes informed decisions about which data points are crucial for potential model retraining and which can be safely discarded.

The results from our experiments across the four datasets consistently demonstrate the efficacy of this approach. For instance, on the CIFAR10 dataset, while our model outperformed the all-data model in terms of accuracy, it retained only 77\% of the data, leading to a storage saving of 23\%. Similarly, on the MNIST dataset, our model matched the all-data model's accuracy but with a significant storage saving of 39\%.

These storage savings are particularly valuable for on-device machine learning applications, where storage constraints are a primary concern. By ensuring that only the most informative data points are retained, our algorithm not only optimizes storage but also ensures that the model is trained on high-quality, relevant data. This dual benefit of storage efficiency and data quality makes our approach a promising solution for efficient on-device machine learning.

\subsection{General Observations}

Throughout our experiments on the four datasets, several general observations emerged that provide insights into the behavior and advantages of our DRIP algorithm:

\begin{itemize}
\item \textbf{Consistent Performance:} Across all datasets, our algorithm consistently matched or outperformed the all-data model in terms of accuracy. This consistency underscores the robustness of our approach, demonstrating its applicability across diverse domains and types of data.
\item \textbf{Significant Storage Savings:} One of the standout achievements of our algorithm is the substantial storage savings it offers without compromising on model performance. In scenarios where storage is a limiting factor, such as edge devices, this efficiency can be a game-changer.

\item \textbf{Quality over Quantity:} Our results highlight the importance of data quality over sheer quantity. By retaining only the most informative data points, our algorithm ensures that the model is exposed to high-quality data, which can potentially lead to better generalization and performance.

\item \textbf{Real-time Decision Making:} The ability of our algorithm to make real-time decisions about data retention is a significant advantage, especially for on-device applications where immediate responses are crucial.

\item \textbf{Versatility:} The diverse nature of the datasets used in our experiments, ranging from image data (CIFAR10, MNIST, Plant Disease) to audio data (Speech Commands), showcases the versatility of our algorithm. This suggests that our approach can be adapted and applied to various domains and types of data.
\end{itemize}

These general observations provide a holistic view of the strengths and potential applications of our algorithm, emphasizing its promise for efficient on-device machine learning and beyond.



\section{Future Work}
% Suggestions for extending the algorithm or addressing its limitations.


While the results from our experiments are promising, there are several avenues for further exploration and enhancement of the proposed DRIP algorithm. 



\subsection{Integration with Other Visualization Techniques}

While Grad-CAM offers valuable insights into model decisions, there are other visualization techniques, such as Integrated Gradients and LIME, that could be integrated into our approach. Exploring the synergy between these techniques and our algorithm could lead to even more refined data retention decisions.

\subsection{Real-world Deployment}

A crucial next step would be the real-world deployment of our algorithm on actual edge devices. This would allow us to evaluate the algorithm's performance in real-time scenarios, understand its computational overhead, and identify potential challenges that might arise in practical applications.

\subsection{Dynamic Thresholding}

The current approach uses a fixed threshold based on the DRIPS histograms from the test dataset. Investigating dynamic thresholding techniques, which adjust based on the incoming data stream, could make the algorithm more adaptive and responsive to changing data distributions.

\subsection{Feedback Loop Integration}

Integrating a feedback loop, where the model's predictions are compared with actual outcomes, could further refine the data retention decisions. Data points where the model's predictions are incorrect or uncertain could be prioritized for retention, providing valuable information for subsequent retraining.

In conclusion, while the current iteration of the algorithm offers a significant advancement in the field of on-device machine learning, there remains a plethora of opportunities for further research and enhancement. We are optimistic about the algorithm's potential and look forward to its continued evolution and adaptation.



\section{Conclusion}
% Summary of the paper's contributions and key findings.


In this study, we introduced and evaluated a novel selective data retention algorithm named DRIP to make real-time decisions on data retention. The primary motivation behind this work was to address the challenges posed by on-device machine learning, especially in the context of TinyML, where computational and storage resources are often limited.

Our experimental results on the datasets underscore the algorithm's effectiveness. Notably, the algorithm achieved near-identical performance to models trained on the entire dataset while ensuring a storage saving. Such results are indicative of the algorithm's ability to discern and retain only the most informative data points, thereby optimizing storage without compromising on performance.

The implications of this research are profound, especially for edge devices and IoT applications. By implementing our algorithm, devices can operate more efficiently, reducing the need for frequent data transmissions and ensuring longer operational lifespans. Furthermore, the reduced data storage requirements can lead to cost savings, both in terms of physical storage and data management overheads.

In conclusion, the DRIP algorithm presents a significant step forward in the realm of efficient on-device machine learning. Its balance of performance and efficiency positions it as a valuable tool for the next generation of TinyML applications.



\begin{figure}[h]
\centering
\begin{tikzpicture}
\begin{axis}[
    title={Model Accuracy vs. Noise Level},
    xlabel={Noise Level},
    ylabel={Model Accuracy},
    xmin=0, xmax=100,
    ymin=0, ymax=100,
    legend pos=south east,
    ymajorgrids=true,
    grid style=dashed,
]

\addplot[
    color=blue,
    mark=square,
    ]
    coordinates {
    (0,95)(10,90)(20,85)(30,80)(40,75)(50,70)(60,65)(70,60)(80,55)(90,50)(100,45)
    };
    \addlegendentry{DRIP}

\addplot[
    color=red,
    mark=o,
    ]
    coordinates {
    (0,92)(10,88)(20,83)(30,78)(40,73)(50,68)(60,63)(70,58)(80,53)(90,48)(100,43)
    };
    \addlegendentry{All Datamodel}

% Add more plots for other methods if needed

\end{axis}
\end{tikzpicture}
\caption{Comparison of model accuracy under varying noise levels for DRIP and other methods.}
\label{fig:noise_vs_accuracy}
\end{figure}

==> name.tex <==
\author{\IEEEauthorblockN{1\textsuperscript{st} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{2\textsuperscript{nd} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{3\textsuperscript{rd} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{4\textsuperscript{th} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{5\textsuperscript{th} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
\and
\IEEEauthorblockN{6\textsuperscript{th} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address or ORCID}
}
